A Static Analysis-based Cross-Architecture Performance Prediction Using Machine Learning

Porting code from CPU to GPU is costly and time-consuming; Unless much time is invested in development and optimization, it is not obvious, a priori, how much speed-up is achievable or how much room is left for improvement. Knowing the potential speed-up a priori can be very useful: It can save hundreds of engineering hours, help programmers with prioritization and algorithm selection. We aim to address this problem using machine learning in a supervised setting, using solely the single-threaded source code of the program, without having to run or profile the code. We propose a static analysis-based cross-architecture performance prediction framework (Static XAPP) which relies solely on program properties collected using static analysis of the CPU source code and predicts whether the potential speed-up is above or below a given threshold. We offer preliminary results that show we can achieve 94% accuracy in binary classification, in average, across different thresholds

==> Makefile <==
RM     := /bin/rm -rf

all: 
	pdflatex main
	bibtex main
	sed -e"s/\\\\bibitem/\\\\vspace{-0.09in}\\\\bibitem/g" < main.bbl | sed -e "s/\\\\begin{thebibliography}{10}/\\\\begin{thebibliography}{10}\\\\vspace{-0.001in}/g" > foo; mv foo main.bbl;
	pdflatex main
	pdflatex main

nobib: 
	latex main ; latex main; latex main; dvips  -G0 -o paper.ps -e 0 main; pst2pdf14 paper.ps

clean: 
	$(RM) *.dvi paper.ps *.log *.aux *.pdf *.blg *.bbl *~* main.out



==> abstract_old.tex <==

\begin{abstract}
%GPUs have become ubiquitous, and yet their programming remains
%challenging. One important problem in GPU code development is that it
%is time consuming to develop high-performance code. Moreover, until
\urmish{Parallelizing a sequential program is challenging and time consuming;

Unless much time is invested in development and optimization, 
it is not obvious, a priori, how much speedup is achievable and if it is worth spending time.
In this paper, we develop a binary classifier for predicting parallel performance on a given parallel hardware, 
by analyzing its sequential single-threaded implementation.}

\urmish{Our paper combines two
ideas: (1) Use of static analysis to estimate dynamic
program properties from single-threaded CPU code. (2)
Use of machine learning to develop a
model that captures the correlation between static program properties of the single-threaded CPU implementation and performance of parallel implementation.}

\urmish{For evaluation, we use GPU as a parallel target hardware.
We define 10 statically determinable program properties and show
that an ensemble classifier (random forest) can classify the speedup of GPU over single-threaded CPU implementation into XXX classes with XXX accuracy. We show our technique is robust across different speedup cutoffs and different platforms.}

\nurmish{Developing high-performance parallel program is challenging and time consuming. Its hard to comprehend the speed-up opportunities after parallelization of a sequential program and to figure out the right algorithm to get those speed-up benefits. In this paper, we show how to predict speed-up of a sequential code on a parallel hardware using statically determined properties of a sequential code. We show how to determine these features and pre-process them. Finally, we show how to use Random Forest Decision Tree to capture the relationship between these static properties and the speed-up after parallelization. Further, we can use this framework to guide a programmer to chose the set of algorithms that can best achieve the predicted speed-up. We evaluate our idea by predicting speed-up on a GPU platform. We are able to achieve 94\% accuracy for predicting speed-up between the range XXX-XXX. We believe this tool can be extremely useful as a feature in an IDE to assist developers or to guide a reinforcement learning algorithm for device placement optimization.}
\end{abstract}


==> fig/insight.tex <==
\begin{figure}[t]
  \begin{center}
   \includegraphics[width=0.75\linewidth]{fig/insight3.pdf}
   %\rule{5cm}{3cm}
  \end{center}
  \caption{The single tree that approximates the random forest model which predicts speedup range with (5,20) cutoffs.}
  \label{fig:insight}
  \vspace{-0.25 in}
\end{figure}



==> fig/overview.tex <==
\begin{figure}
  \begin{center}
   \includegraphics[width=0.65\linewidth]{fig/workflow.pdf}
 \end{center}
  \vspace{-0.10in}
  \caption{Overall flow}
  \label{fig:overview}
  \vspace{-0.2in}
%\vspace{-0.2in}
\end{figure}



==> fig/rf.tex <==
\begin{figure}[t!]
  \begin{center}
  \includegraphics[width=\linewidth]{fig/rfpdf.pdf}
%\rule{5cm}{3cm}
  \end{center}
  \vspace{-0.05in}
  \caption{Model construction overview}
  \vspace{-0.18in}
  \label{fig:rf}
\end{figure}


==> fig/tree.tex <==
\begin{figure}[t]
  \begin{center}
  \includegraphics[width=\linewidth]{fig/tree.pdf}
%\rule{5cm}{3cm}
  \end{center}
  \caption{An instance of a learned tree}
  \label{fig:tree}
\end{figure}


==> graph/branch-speedup.tex <==
\begin{figure}[t]
  \begin{center}
  %\includegraphics[width=\linewidth]{graph/staticAnalysis-sweepBranch/sweepbranch.pdf}
\rule{5cm}{3cm}
  \end{center}
  \captionsetup{justification=centering}
  \vspace{-0.07in}
  \caption{Speedup prediction sensitivity to branch ratio.}
  \label{fig:branch-speedup}
  \vspace{-0.19in}
\end{figure}


==> graph/loop-speedup.tex <==
\begin{figure}[t]
  \begin{center}
  %\includegraphics[width=\linewidth]{graph/staticAnalysis-sweepBranch/sweepbranch.pdf}
	\rule{5cm}{3cm}
  \end{center}
  \captionsetup{justification=centering}
  \vspace{-0.07in}
  \caption{Speedup prediction sensitivity to loop trip count.}
  \label{fig:loop-speedup}
  \vspace{-0.19in}
\end{figure}


==> graph/precision-backup.tex <==
\begin{figure}
		\begin{center}
		\begin{framed}
		\includegraphics[width=\linewidth]{graph/precision.pdf}
		\newline
                \setlength{\tabcolsep}{.3em}
		\vspace*{0 cm}
		\newline
		\footnotesize
		\renewcommand{\arraystretch}{1.5}
		\begin{tabular}{cccccc}
		\cmidrule[1pt]{3-6}
		\multicolumn{1}{l}{}				 &   & \multicolumn{4}{c}{Number of intervals} \\\cmidrule[1pt]{3-6}
		\multicolumn{1}{l}{}         &   & \multicolumn{1}{c}{3} & \multicolumn{1}{c}{4} & \multicolumn{1}{c}{5} & \multicolumn{1}{c}{6} \\\cmidrule[1pt]{2-6}
		\multicolumn{1}{c}{\multirow{5}{*}{\adjustbox{angle=90}{Cutoffs}}}& $x_1$ & (3,10,1)  	& (3,10,1) 	& (3,10,1) 		& (3,10,1)\\%\cline{2-2}
		\multicolumn{1}{c}{} & $x_2$ & (10,100,5)	& (10,50,5)	& (10,50,5)		& (10,40,5)\\%\cline{2-2}
		\multicolumn{1}{c}{} & $x_3$ & - 			& (20,100,5)& (20,70,10)	& (20,60,10)\\%\cline{2-2}
		\multicolumn{1}{c}{} & $x_4$ & -			& -			& (30,100,10)	& (30,80,10)\\%\cline{2-2}
		\multicolumn{1}{c}{} & $x_5$ & -			& -			& -			& (40,100,10)\\\cmidrule[1pt]{2-6}
		%\multicolumn{2}{|l|}{\# Models}  & 152  & 1224      & 3456          &  11760 \\\hline
		\end{tabular}
		\end{framed}
		\end{center}
		  %\captionsetup{justification=left}
		  \caption{The figure shows the accuracy-precision tradeoff. The Table below shows the space range that each bar represents. 
			$(l,u,s)$ at row $i$ and column $j$ shows that cutoff $x_i$ for $j$ intervals sweeps between $l$ and $u$ in steps of $s$.}
		  \label{fig:precision}
                  \vspace{-0.15in}
\end{figure}


==> graph/stability-platform1.tex <==
\begin{figure*}
  \begin{center}
  \includegraphics[width=\linewidth]{graph/stability.pdf}
  \end{center}
  \captionsetup{justification=centering}
  \vspace{-0.2in}
  \caption{Prediction accuracy for different speedup intervals. $(x,y)$ represents two speedup cutoffs at x and y, i.e. speedup range is divided into $(0,x]$, $(x,y]$, and $(y,\infty)$. For clarity only a subset of axis-labels are shown. Between the shown axis-labels, the y increments by steps of 5 up to 100.}
  \label{fig:stability}
  \vspace{-0.2in}
\end{figure*}


==> graph/stability-platform2.tex <==
\begin{figure*}
  \begin{center}
  \includegraphics[width=\linewidth]{graph/stability-platform2pdf.pdf}
  \end{center}
  \captionsetup{justification=centering}
  \vspace{-0.2in}
  \caption{Prediction accuracy for different speedup intervals. $(x,y)$ represents two speedup cutoffs at x and y, i.e. speedup range is divided into $(0,x]$, $(x,y]$, and $(y,\infty)$. For clarity only a subset of axis-labels are shown. Between the shown axis-labels, the y increments by steps of 5 up to 100.}
  \label{fig:stability-platform2}
  \vspace{-0.2in}
\end{figure*}


==> intro_old.tex <==
\section{Introduction}\label{sec:intro}
\urmish{\paragraph{Motivation}}
\urmish{Porting code from CPU to GPU is a very slow and tedious process, with no
promise of success.  The programmer should think about how to extract
and restructure the parallelism in the CPU code, how to explicitly
manage and map to GPU memory hierarchy, and various other intricate
details of how the program and GPU hardware interact.  If desired speedup is
not achieved at the end of this process, time and effort will go
wasted.  The goal of this paper is to \textit{quickly} and
\textit{accurately} predict the speedup interval achievable on GPUs by
analyzing the CPU source code.}
\paragraph{Motivation}
\nurmish{Porting code from CPU to GPU is a very slow and tedious process, with a likelihood of failure. A programmer needs to reshape the existing CPU code to extract maximum parallelism, learn how to map the data-structures to GPU memory hierarchy and needs to be constantly aware of multiple hardware specific properties like \#streaming cores etc. Restructuring code to incorporate these aspects of the platform is extremely time consuming and these efforts come without any guarantee of success. Thus, a tool that can \textit{quickly} and
\textit{accurately} predict the speed-up interval achievable on GPUs by
analyzing the CPU source code could be extremely useful to democratize GPU development to the masses.}

%\footnote{Some may posit that programmers
%  can estimate speedup from intuition. Others have shown
%  pitfalls of relying on intuitions like branch divergence is
%  detrimental to speedup, or memory coalescing is beneficial, etc.
%There are three problems with these heuristics: 
%(1) There is no intuition on how these individual intuitions combine; in other words, it is not clear which factor is stronger when multiple positive and negative factors exist.
%(2) How these program properties interact depends on the underlying hardware.
%(3) The intuitions on the direction of impact are sometimes false.}
%To give an example, the common belief that branch divergence has negative impact on speedup is not always true.
%Branch divergence on GPU and branch unpredictability on CPU are often times correlated. 
%However, there are cases where branch unpredictability hurts CPU performance more than the branch divergence hurts GPU performance,
%and the overall direction of impact is positive.}.

\paragraph{State-of-the-art Tools}
Our work belongs in the broad paradigm of cross-architecture
performance prediction: predicting performance of one architecture
using an implementation from another
architecture~\cite{saavedra1996analysis,lau2005strong,annavaram2004fuzzy,Hoste06performanceprediction}.
%Techniques under this paradigm can be compared along
%two axes,
%prediction precision and prediction speed, as shown in Table~\ref{table:related}. 
%Broadly, they can be categorized into two categories based on their measurement of program properties:
%(1) \emph{execution-based} and (2) 
%\emph{human-based}.
Techniques under this paradigm belong in two broad categories:
(1) \emph{execution-based} measurement of program properties and (2) 
\emph{human-based} estimation of program properties.

\begin{table*}[tbp]
\centering
\small
%\footnotesize
%\def\arraystretch{0.87}
\setlength{\tabcolsep}{.25em}
\begin{tabular}{>{\RaggedRight}p{0.25in}>{\RaggedRight}p{0.95in}>{\RaggedRight}p{0.70in}>{\RaggedRight}p{0.55in}>{\RaggedRight}p{0.4in}>{\RaggedRight}p{2.2in}>{\RaggedRight}p{1.6in}} \hline

Year & Related Work           & Feature & Prediction & Prediction & \multicolumn{1}{c}{Usage} & Drawback \\ 
 &           &  Measurement & \textbf{Precision} & \textbf{Runtime} & &  \\ \hline
1996 & AbOps model\cite{saavedra1996analysis} & Execution & High & Slow & Performance across Cray, MIPS, SPARC & \emph{Works for ``simple'' machines} \\
2006 & Hoste et. al.\cite{Hoste06performanceprediction} & Execution & Low & Slow & SPEC rank across x86, SPARC, PowerPC &  \emph{CPU-style machines only} \\
2009 & Roofline\cite{Williams:2009:RIV:1498765.1498785,boat-hull0}     & Human                   & Very Low & Slow &  Upper-bound speedups  &  \emph{Not general; human-intensive}                         \\
2011 & Grophecy\cite{meng2011grophecy}   & Human                           & High  & Slow & GPU Speedup prediction  &  \emph{Not general; human-intensive}         \\
2013 & Meswani et. al.\cite{meswani2013modeling}               & Execution                           & Low & Slow & Idiom-based projections & \emph{Not general} \\
2014 & Baldini et. al.\cite{baldini2014predicting}                & Execution                           & Low & Slow & Speedup classification as hi/lo & \emph{Requires OpenMP code}                              \\
2015 & XAPP\cite{ardalani}               & Execution                           & Very High & Slow & GPU numerical speedup from CPU-code & \emph{Hours/days measurement time}                       \\
    2016 & \textbf{This paper}             & Source code                         & Medium & Fast & GPU range-speedup from CPU-code & ?                             \\ \hline
\end{tabular}
%$\dagger$Performance is weighted sum of occurrence frequency of compound operators 
\caption{Relationship to related work}
\vspace{-0.15in}
\label{table:related}
\end{table*}

\emph{$\bullet$ Execution-based} techniques rely on dynamic binary
instrumentation to obtain program properties, which introduce 10$\times$ to 1000$\times$ slowdown.
Features collected
are fed into a performance
model, analytical model, or machine-learning engine
to obtain performance on the target architecture.
\dnewsha{Saavedra and Smith~\cite{saavedra1996analysis}
pioneered this paradigm and developed a ``linear'' model.  They
develop an abstract machine model that consists of a set of abstract
operations representing %, for some particular programming language, 
the basic operators and language constructs present in programs. A special
benchmark, called a machine characterizer, is used to measure
experimentally the time it takes to execute each abstract operation
(AbOp). Frequency counts of AbOps are obtained by instrumenting and
running benchmarks.  The machine and program characterizations are
then combined 
%(essentially a weighted sum of occurrence frequencies of
%each AbOp in the program of interest) 
to obtain execution-time
predictions.
%\footnote{Lightly paraphrased from original paper.} 
When
features interact, like in today's complex machines, their approach
falls short.  
}
A general technique was proposed by Hoste
et. al.~\cite{Hoste06performanceprediction} to predict SPEC ranking
across several ISAs, like X86, SPARC, and PowerPC.  
Baldini et. al. ~\cite{baldini2014predicting} extended this paradigm to find the best
GPU platform based on OpenMP programs. 
Ardalani et. al. ~\cite{ardalani} proposed XAPP, an adaptation
of~\cite{Hoste06performanceprediction}, by changing the
target ISA to NVIDIA's GPU ISAs.
XAPP predicts the exact value of speedup with 27\% relative error.
However, it can take anywhere between minutes to days to predict the exact speedup value. 

We are interested in a speedup prediction framework that can be embedded
within the integrated development environments (IDEs), which can
\emph{interactively} provide developers with feedback
on potential performance improvements gained by
porting fragments of their single-threaded code to a GPU.
This imposes new constraints on the cross-architecture performance prediction paradigm:
the run-time overhead should be less than seconds.
However, the execution-based approaches are too slow to meet this requirement
---they rely on dynamic binary instrumentation to
obtain the precise value of each feature.
If we can eliminate dynamic binary instrumentation
and obtain program properties statically, we can
considerably reduce the overhead.
%however not all
%program properties are collectible statically. 
%Besides, it is hard to get the precise values of each feature statically.
%It is an open question whether the statically collectible features are sufficient to predict the speedup.

\emph{$\bullet$Human-based} The human-based approach avoids the
  binary-instrumentation overhead and instead uses humans to estimate
  features. Roofline-based
  approaches~\cite{Williams:2009:RIV:1498765.1498785} use program
  properties to estimate an upper-bound on
  speedup. These
  human-intensive tasks are slow and imprecise.

Table~\ref{table:related} compares the related work along two axes, the prediction precision accuracy and prediction runtime overhead.
As shown, we are the only technique that can quickly predict the speedup with sufficient precision.
\paragraph{Problem statement}
We introduce a novel sub-branch to the cross-architecture performance
prediction paradigm: \emph{Intermediate-representation(IR)-based} feature estimation.
Our approach achieves the best of both worlds: 
it avoids human involvement and
slowdowns of binary instrumentation. Our paper makes the insightful
observation that program properties obtainable 
with simple static analysis---without execution---% 
are sufficiently explanatory to
predict cross-architecture performance.
Regardless of whether
programmers consider the execution-time and human-time overheads of
existing tools a barrier for their usage, from an aesthetic and
intellectual standpoint, the limit of static analysis for this problem
is an open question. Furthermore, a source-code-based technique opens
up the possibility of embedding such fast estimates into IDEs.

\input{fig/overview.tex}
\paragraph{Insight} 
We investigate and propose program feature extraction
via static analysis of CPU code, with the goal of predicting GPU
performance using machine learning.  In particular, we 
statically extract numerical features from programs.
We then use a machine-learning-based
discretizer to turn numerical features into categorical ones.
Finally, we employ the \emph{random forest
  classification} technique to predict the \emph{speedup range}. Two
inter-related key insights enable us to use source-code analysis to
obtain meaningful program properties.  Figure~\ref{fig:overview} shows
the overall flow of our work.

While IR analysis can only provide approximate values of
program features---since it lacks information on the influence of
dynamic effects---we observe that the approximate values of features can
be made accurate by reducing precision. In particular, we reduce the
feature precision to just one bit---\emph{high} or \emph{low}. In practice,
we observe that static analysis is 100\% accurate in determining the binary values of 
the program properties. 
We have discovered a meaningful set of ten features
that are statically collectible. We use machine learning here to
determine where to place cut-points on any given feature to discretize
it as high or low.
Second, we observe that binary feature inputs
are sufficiently explanatory to predict the range of speedup. In particular, by using a
classification-based machine learning technique, we classify
speedup range into as many as 5 intervals
(e.g. $[0,3)$, $[3, 20)$, $[20, 50)$, $[50, 100)$, $[100, \infty)$),
in less than a second.
We let users to provide the speedup intervals.

%Demonstrating the idea
%      that very low-precision inputs are sufficient to develop a
%      classification technique that predicts the speedup range is the
%      third contribution of our work.

\paragraph{Practical implementation}
We use a set of 147 single-threaded CPU programs (written in C or C++)
that are already ported into GPU code (written in CUDA) to construct
and evaluate our model. 
In an offline and one-time training phase
(per GPU platform), we collect program properties from CPU
codes and GPU performance from GPU codes within our training set, 
and learn the correlation between features and
speedup on GPU.
For any new program, we use static analysis to obtain binary feature vectors.
Therefore, we train our machine learning technique with binary feature values.
We use the feature matrix provided by Ardalani et. al., but since their features are in continuous form,
we have to discretize them into
binary values before feeding into our machine learning technique. 
We use random forest technique to predict the range of speedup. 
We discretize speedup into ranges based on the user
preference. Our prediction accuracy is 94\% for the interesting speedup
intervals of $\emph{speedup} \leq 3$
and $3 < \emph{speedup}$. 
Figure~\ref{fig:stability}
shows that our model accurately predict speedup for different speedup cutoffs.

\paragraph{Contributions}
This paper makes one broad intellectual contribution: We observe and
demonstrate that statically determinable program properties are
sufficient to predict GPU performance. Specifically, 
(1) we identify and
precisely define 10 program properties that are accurately statically
determinable and are sufficiently explanatory (from a machine
learning perspective); 
(2) we determine a method for converting the
approximate static estimates into an accurate low-precision value; 
and (3) we implement a machine-learning classification method that uses
random forests to predict speedup range.
%\aws{``makes'' above is weird}
% In practical terms, we release a suite of
%benchmarks with CPU/GPU code regions that allows anyone to replicate
%and use our tool, and we will release our ML tools as a read



%The decision to port a CPU code to GPU is often times made based on the speedup range rather than the actual speedup value.
%However, different programmers make their decisions based on different speedup ranges.
%One programmer might find speedup greater than 5 promising, while another programmer finds 20 the minimum threshold to invest her time.
%This difference comes from the diversity in CPU/GPU expertise, time and human resource availability, 
%the importance degree of the performance of the program, and the capability of the host CPU platform and the target GPU platform.  
%Therefore, we allow the user to specify the number of intervals and intervals.


==> tables/accuracy.tex <==
\begin{table}
\center
\tabcolsep=0.05cm
\begin{tabular}{lcc@{\hskip 0.1in}|@{\hskip 0.1in}lcc}\hline
Benchmarks&Meas.&Pred.&Benchmarks&Meas.&Pred.\\\hline
fft2-1-other & L & L & bfs0-mv2-2-ls & H & H \\
\cellcolor{lightgray}pf1-1-rd & \cellcolor{lightgray}L & \cellcolor{lightgray}M & bfs0-mv4-2-ls & H & H \\
four1-1-$\mu$ & L & L & bfs2-mv2-2-ls & H & H \\
four2-1-$\mu$ & L & L & euler3d2-1-rd & H & H \\
four3-1-$\mu$ & L & L & nn1-mv0-1-rd & H & H \\
four4-1-$\mu$ & L & L & nn1-mv1-1-rd & H & H \\
four5-1-$\mu$ & L & L & nn1-mv2-1-rd & H & H \\
four6-1-$\mu$ & L & L & nn1-mv3-1-rd & H & H \\
four7-1-$\mu$ & L & L & one11-1-$\mu$ & H & H \\
four8-1-$\mu$ & L & L & one11-2-$\mu$ & H & H \\
four9-1-$\mu$ & L & L & one11-3-$\mu$ & H & H \\
sp1-mv0-1-ls & L & L & one1-1-$\mu$ & H & H \\
backprop2-1-rd & M & M & one12-1-$\mu$ & H & H \\
bfs0-mv0-1-ls & M & M & one1-2-$\mu$ & H & H \\
bfs0-mv0-2-ls & M & M & one1-3-$\mu$ & H & H \\
bfs0-mv6-2-ls & M & M & one2-1-$\mu$ & H & H \\
bfs2-1-rd & M & M & one2-2-$\mu$ & H & H \\
bfs2-mv0-2-ls & M & M & one2-3-$\mu$ & H & H \\
bfs2-mv1-2-ls & M & M & one3-1-$\mu$ & H & H \\
bfs2-mv3-2-ls & M & M & one5-1-$\mu$ & H & H \\
bfs2-mv4-2-ls & M & M & one5-2-$\mu$ & H & H \\
bfs2-mv5-2-ls & M & M & one5-3-$\mu$ & H & H \\
bfs2-mv6-2-ls & M & M & sp0-mv2-2-ls & H & H \\
bfs2-mv8-2-ls & M & M & sp0-mv3-2-ls & H & H \\
bfs2-mv9-2-ls & M & M & sp0-mv6-2-ls & H & H \\
b+tree1-1-rd & M & M & sp0-mv9-2-ls & H & H \\
b+tree2-1-rd & M & M & sp1-mv2-2-ls & H & H \\
euler3d1-1-rd & M & M & sp1-mv3-2-ls & H & H \\
euler3d4-1-rd & M & M & \cellcolor{lightgray}sp1-mv4-2-ls & \cellcolor{lightgray}H & \cellcolor{lightgray}L \\
ftv20-1-others & M & M & sp1-mv5-2-ls & H & H \\
ftv24-1-others & M & M & sp1-mv6-2-ls & H & H \\
ftv26-1-others & M & M & sp1-mv7-2-ls & H & H \\
ftv27-1-others & M & M & \cellcolor{lightgray}sp1-mv8-2-ls & \cellcolor{lightgray}H & \cellcolor{lightgray}L \\
one6-1-$\mu$ & M & M & sp1-mv9-2-ls & H & H \\
one6-2-$\mu$ & M & M & sp2-mv1-2-ls & H & H \\
one6-3-$\mu$ & M & M & sp2-mv2-2-ls & H & H \\
one9-1-$\mu$ & M & M & sp2-mv3-2-ls & H & H \\
sp0-mv1-2-ls & M & M & sp2-mv4-2-ls & H & H \\
\cellcolor{lightgray}srad\_v13-1-rd & \cellcolor{lightgray}M & \cellcolor{lightgray}H & sp3-mv3-2-ls & H & H \\
\cellcolor{lightgray}srad\_v14-1-rd & \cellcolor{lightgray}M & \cellcolor{lightgray}H & sp3-mv4-2-ls & H & H \\
\cellcolor{lightgray}srad\_v22-1-rd & \cellcolor{lightgray}M & \cellcolor{lightgray}H & sp3-mv5-2-ls & H & H \\
sssp0-mv0-1-ls & M & M & sp3-mv7-2-ls & H & H \\
sssp0-mv0-2-ls & M & M & sp3-mv9-2-ls & H & H \\
sssp0-mv7-2-ls & M & M & srad\_v11-1-rd & H & H \\
sssp0-mv8-2-ls & M & M & srad\_v15-1-rd & H & H \\
sssp2-mv0-1-ls & M & M & sssp2-mv2-2-ls & H & H \\
sssp2-mv0-2-ls & M & M & \cellcolor{lightgray}sssp2-mv4-2-ls & \cellcolor{lightgray}H &\cellcolor{lightgray} L \\
sssp2-mv1-2-ls & M & M & three1-1-$\mu$ & H & H \\
sssp2-mv8-2-ls & M & M & two2-1-$\mu$ & H & H \\
sssp2-mv9-2-ls & M & M &&&\\\hline
\multicolumn{3}{l}{\textbf{Accuracy}}	   &\multicolumn{3}{l}{\textbf{93\%}} \\\hline	
\end{tabular}
\vspace{0.2in}
\caption{Speedup range prediction accuracy for following speedup ranges: low (speedup $\leq$ 3), medium (3 $<$ speedup $\leq$ 20) and high speedup (speedup $>$ 20).}\label{table:accuracy}
\vspace{-0.2in}
\end{table}


==> tables/platform-bl.tex <==
\begin{table}
\small
\center
\begin{tabular}{lll}\toprule
 & \textbf{GPU Platform} & \textbf{CPU Platform}\\ \midrule
Micro\-architecture & Maxwell & Core-i7 \\ 
Model & GTX 750 & i7-2600 \\ 
\# SMs & 7 & -  \\
\# cores per SM & 192 & - \\
Core freq. & 1.32 GHz & 3.4 GHz \\
Memory freq./bandwidth & 2.5 GHz &  21 GB/s \\ \midrule
\end{tabular}
\vspace{-0.1in}
\caption{Hardware platforms pecifications.}\label{table:platform}
\end{table}



==> tables/thacc2.tex <==
\begin{table}
\center
\tabcolsep=0.05cm
\footnotesize
\begin{tabular}{lcc@{\hskip 0.1in}|@{\hskip 0.1in}lcc|@{\hskip 0.1in}lcc}\hline
Benchmarks&Meas.&Pred.&Benchmarks&Meas.&Pred.&Benchmarks&Meas.&Pred.\\\hline
backprop2-1-rd & L & L & srad\_v22-1-rd & L & L & one5-3-$\mu$ & H & H \\
bfs0-mv0-1-ls & L & L & sssp0-mv0-1-ls & L & L &  one7-1-$\mu$ & H & H \\
bfs0-mv0-2-ls & L & L & sssp0-mv0-2-ls & L & L &  one8-1-$\mu$ & H & H \\
bfs0-mv5-2-ls & L & L & \cellcolor{lightgray}sssp0-mv1-2-ls & \cellcolor{lightgray}L & \cellcolor{lightgray}H & raycasting1-1-capp & H & H \\
bfs0-mv6-2-ls & L & L & \cellcolor{lightgray}sssp0-mv3-2-ls & \cellcolor{lightgray}L & \cellcolor{lightgray}H & sp0-mv2-2-ls & H & H \\
bfs2-1-rd & L & L & sssp0-mv7-2-ls &  L & L & sp0-mv3-2-ls & H & H \\
bfs2-mv0-1-ls & L & L & sssp0-mv8-2-ls & L & L & sp0-mv4-2-ls & H & H \\
bfs2-mv0-2-ls & L & L & sssp0-mv9-2-ls & L & L & sp0-mv6-2-ls & H & H \\
bfs2-mv1-2-ls & L & L & sssp2-mv0-1-ls & L & L & sp0-mv8-2-ls & H & H \\
bfs2-mv3-2-ls & L & L & sssp2-mv0-2-ls & L & L & sp0-mv9-2-ls & H & H \\
bfs2-mv4-2-ls & L & L & sssp2-mv1-2-ls & L & L & sp1-mv2-2-ls & H & H \\
bfs2-mv5-2-ls & L & L & sssp2-mv7-2-ls & L & L & sp1-mv3-2-ls & H & H \\
bfs2-mv6-2-ls & L & L & sssp2-mv8-2-ls & L & L & sp1-mv4-2-ls & H & H \\
bfs2-mv8-2-ls & L & L & sssp2-mv9-2-ls & L & L & sp1-mv5-2-ls & H & H \\
bfs2-mv9-2-ls & L & L & two3-1-$\mu$ & L & L & sp1-mv6-2-ls & H & H \\
b+tree1-1-rd & L & L & two4-1-$\mu$ & L & L & sp1-mv7-2-ls & H & H \\
b+tree2-1-rd & L & L & ftv1-1-other & L & L & sp1-mv8-2-ls & H & H \\
euler3d1-1-rd & L & L & bfs0-mv1-2-ls &  H &  H & sp1-mv9-2-ls & H & H \\
euler3d4-1-rd & L & L & bfs0-mv2-2-ls & H & H & sp2-mv1-2-ls & H & H \\
fft1-1-capp & L & L & bfs0-mv3-2-ls & H & H & sp2-mv2-2-ls & H & H \\
fft2-1-capp & L & L & bfs0-mv4-2-ls & H & H & sp2-mv3-2-ls & H & H \\
ftv0-1-other & L & L & bfs0-mv7-2-ls & H & H & sp2-mv4-2-ls & H & H \\
ftv4-1-other & L & L & bfs0-mv9-2-ls & H & H & sp2-mv7-2-ls & H & H \\
ftv6-1-other & L & L & \cellcolor{lightgray}bfs2-mv2-2-ls & \cellcolor{lightgray}H & \cellcolor{lightgray}L & sp2-mv8-2-ls & H & H \\
ftv7-1-other & L & L & bfs2-mv7-2-ls & H & H & sp2-mv9-2-ls & H & H \\
one6-1-$\mu$ & L & L & convolution1-1-capp & H & H & sp3-mv2-2-ls & H & H \\
one6-2-$\mu$ & L & L & euler3d2-1-rd & H & H & sp3-mv3-2-ls & H & H \\
one6-3-$\mu$ & L & L & nn0-1-rd & H & H & sp3-mv4-2-ls & H & H \\
one9-1-$\mu$ & L & L & nn1-1-rd & H & H & sp3-mv5-2-ls & H & H \\
\cellcolor{lightgray}particle\_filter1-1-rd & \cellcolor{lightgray}L & \cellcolor{lightgray}H & nn2-1-rd & H & H & sp3-mv6-2-ls & H & H \\
four6-1-$\mu$ & L & L & montecarlo1-1-capp & H & H & sp3-mv7-2-ls & H & H \\
\cellcolor{lightgray}four2-1-$\mu$ & \cellcolor{lightgray}L & \cellcolor{lightgray}H & montecarlo2-1-capp & H & H & sp3-mv8-2-ls & H & H \\
four8-1-$\mu$ & L & L & nn3-1-rd & H & H & sp3-mv9-2-ls & H & H \\
four9-1-$\mu$ & L & L & one10-1-$\mu$ & H & H & srad\_v11-1-rd & H & H \\
four10-1-$\mu$ & L & L & one11-1-$\mu$ & H & H & srad\_v15-1-rd & H & H \\
four3-1-$\mu$ & L & L & one11-2-$\mu$ & H & H & sssp0-mv2-2-ls & H & H \\
\cellcolor{lightgray}four4-1-$\mu$ & \cellcolor{lightgray}L & \cellcolor{lightgray}L & one11-3-$\mu$ & H & H & sssp0-mv4-2-ls & H & H \\
four5-1-$\mu$ & L & L & one1-1-$\mu$ & H & H & sssp0-mv5-2-ls & H & H \\
four7-1-$\mu$ & L & L & one12-1-$\mu$ & H & H & sssp2-mv2-2-ls & H & H \\
sp0-mv1-2-ls & L & L & one1-2-$\mu$ & H & H & sssp2-mv3-2-ls & H & H \\
\cellcolor{lightgray}sp1-mv0-1-ls & \cellcolor{lightgray}L & \cellcolor{lightgray}H & one13-1-$\mu$ & H & H & sssp2-mv4-2-ls & H & H \\
sp1-mv0-2-ls & L & L & one1-3-$\mu$ & H & H &  sssp2-mv5-2-ls & H &  H \\
sp2-mv0-1-ls & L & L & one2-1-$\mu$ & H & H & sssp2-mv6-2-ls & H & H \\
\cellcolor{lightgray}sp2-mv0-2-ls & \cellcolor{lightgray}L & \cellcolor{lightgray}H & one2-2-$\mu$ & H & H & three1-1-$\mu$ & H & H \\
sp2-mv6-2-ls & L & L & one2-3-$\mu$ & H & H & tsearch1-1-capp & H & H \\
sp3-mv0-1-ls & L & L & one3-1-$\mu$ & H & H & two1-1-$\mu$ & H & H \\
\cellcolor{lightgray}sp3-mv0-2-ls & \cellcolor{lightgray}L & \cellcolor{lightgray}H & one4-1-$\mu$ & H & H & two2-1-$\mu$ & H & H \\
srad\_v13-1-rd & L & L & one5-1-$\mu$ & H & H & two5-1-$\mu$ & H & H \\
srad\_v14-1-rd & L & L & one5-2-$\mu$ & H & H & two6-1-$\mu$ & H & H \\\hline
\multicolumn{5}{l}{\textbf{Accuracy}}	   & \multicolumn{4}{l}{\textbf{\%90}} \\\hline	
\end{tabular}
\caption{Speedup range prediction accuracy for following ranges: low speedup (speedup $\leq$ 3), and high speedup (speedup $>$ 3).}\label{table:thacc}
\end{table}


==> tables/xapp-time.tex <==
\begin{table}[]
\centering
\renewcommand{\arraystretch}{1.15}
\begin{tabular}{llllll|}
\cline{2-6}
                                 & \multicolumn{5}{|c|}{ \% of datapoints with overhead in:}                                                                                       \\ \cline{2-6} 
                                 & \multicolumn{1}{|l}{mSec.} & \multicolumn{1}{l}{Sec.} & \multicolumn{1}{l}{Min.} & \multicolumn{1}{l}{Hrs.} & \multicolumn{1}{l|}{Days} \\ \hline
\multicolumn{1}{|l|}{XAPP} &     0\% & 18\%                       &  75\%                          & 6\%                           &              1\%             \\ \hline
\multicolumn{1}{|l|}{This paper} &       100\%  & 0\%                      &  0\%                            & 0\%                           &     0\%                      \\ \hline
\end{tabular}
\caption{Feature measurement overhead comparison between XAPP and our proposal.}\label{table:xapp-time}
\vspace{-0.25in}
\end{table}

